Approximate Computation of Reach Sets in Hybrid Systems

One of the most important problems in hybrid systems is the {\em reachability problem}. The reachability problem has been shown to be undecidable even for a subclass of {\em linear} hybrid systems. In view of this, the main focus in the area of hybrid systems has been to find {\em effective} semi-decision procedures for this problem. Such an algorithmic approach involves finding methods of computation and representation of reach sets of the continuous variables within a discrete state of a hybrid system. In this paper, after presenting a brief introduction to hybrid systems and reachability problem, we propose a computational method for obtaining the reach sets of continuous variables in a hybrid system. In addition to this, we also describe a new algorithm to over-approximate with polyhedra the reach sets of the continuous variables with linear dynamics and polyhedral initial set. We illustrate these algorithms with typical interesting examples.

==> junk/Sec7.tex <==


\section{Discussion and Conclusion}

 An important issue of hybrid systems appears to be 
 computability of the reach sets of the continuous variables.
 In this context, approximation of the reach sets by more
 convenient sets, such as polyhedra and ellipsoids, is discussed 
 in the literature. In this paper, along with a method for
 finding the reach sets, an algorithm for over-approximation
 of the reach sets by polyhedra for linear systems with
 polygonal initial sets is presented. A practical version
 of the over-approximation algorithm is also discussed in
 this paper. However, it seems that better results of
 over-approximation may be obtained by taking the intersection
 of the polyhedron obtained by the method reported here with
 that obtained by the method given in \cite{ABDM00}. It is
 hoped that the over-approximation method presented here
 may be extended to systems with more general dynamics and
 initial sets.


